Double electron capture searches in $^{74}$Se

A search for various double electron capture modes of $^{74}$Se has been performed using an ultralow background Ge-detector in the Felsenkeller laboratory, Germany. Especially for the potentially resonant transition into the 1204.2 keV excited state of $^{74}$Ge a lower half-life limit of $0.70\cdot 10^{19}$ yr (90% credibility) has been obtained. Serious concerns are raised about the validity of obtained $^{74}$Se limits in some recent publications.

==> commands.tex <==
\definecolor{brown}{RGB}{139,69,19}


\newcommand{\nuc}[2]{$^{#2}\rm #1$}

\newcommand{\bb}[1]{$\rm #1\nu \beta \beta$}
\newcommand{\bbm}[1]{$\rm #1\nu \beta^- \beta^-$}
\newcommand{\bbp}[1]{$\rm #1\nu \beta^+ \beta^+$}
\newcommand{\bbe}[1]{$\rm #1\nu \rm ECEC$}
\newcommand{\bbep}[1]{$\rm #1\nu \rm EC \beta^+$}

%\newcommand{\gerda}{\textsc{Gerda}}
\newcommand{\largeGERDA}{{LArGe}}
\newcommand{\PI}{\mbox{\textsc{Phase\,I}}}
\newcommand{\PIa}{\mbox{\textsc{Phase\,Ia}}}
\newcommand{\PIb}{\mbox{\textsc{Phase\,Ib}}}
\newcommand{\PIc}{\mbox{\textsc{Phase\,Ic}}}
\newcommand{\PII}{\mbox{\textsc{Phase\,II}}}

%\newcommand{\geant}{\textsc{GEANT4}}
%\newcommand{\mage}{\textsc{MaGe}}


\newcommand{\nPlus}{\mbox{n$^+$ electrode}}
\newcommand{\pPlus}{\mbox{p$^+$ electrode}}

\newcommand{\aoe}{$A/E$}


\newcommand{\order}[1]{\mbox{$\mathcal{O}$(#1)}}



\newcommand{\pic}[5]{
       \begin{figure}[ht]
       \begin{center}
       \includegraphics[width=#2\textwidth, keepaspectratio, #3]{#1}
       \end{center}
       \caption{#5}
       \label{#4}
       \end{figure}
}

\newcommand{\apic}[5]{
       \begin{figure}[H]
       \begin{center}
       \includegraphics[width=#2\textwidth, keepaspectratio, #3]{#1}
       \end{center}
       \caption{#5}
       \label{#4}
       \end{figure}
}

\newcommand{\sapic}[5]{
       \begin{figure}[P]
       \begin{center}
       \includegraphics[width=#2\textwidth, keepaspectratio, #3]{#1}
       \end{center}
       \caption{#5}
       \label{#4}
       \end{figure}
}


\newcommand{\picwrap}[9]{
       \begin{wrapfigure}{#5}{#6}
       \vspace{#7}
       \begin{center}
       \includegraphics[width=#2\textwidth, keepaspectratio, #3]{#1}
       \end{center}
       \caption{#9}
       \label{#4}
       \vspace{#8}
       \end{wrapfigure}
}


\newcommand{\baseT}[2]{\mbox{$#1\cdot10^{#2}$}}
\newcommand{\baseTsolo}[1]{$10^{#1}$}
\newcommand{\THL}{$T_{\nicefrac{1}{2}}$}


%\newcommand{\cpkyk}{$\rm cts/(kg \cdot yr \cdot keV)$}
\newcommand{\UBI}{$\rm cts/(kg \cdot yr \cdot keV)$}


\newcommand{\Uflux}{$\rm m^{-2} s^{-1}$}
\newcommand{\Ucpd}{$\rm cts/(kg \cdot d)$}
\newcommand{\Uexpo}{$\rm kg \cdot d$}


%\newcommand{\Qbb}{$\rm Q_{\beta\beta}\ $}
\newcommand{\Qbb}{$Q_{\beta\beta}$}



\newcommand{\validate}{\textcolor{blue}{\textit{(validate!!!)}}}

\newcommand{\improve}{\textcolor{blue}{\textit{(improve!!!)}}}

\newcommand{\missing}{\textcolor{red}{\textbf{...!!!...} }}

\newcommand{\quanta}{\textcolor{red}{\textit{(quantitativ?) }}}

\newcommand{\misscite}{\textcolor{red}{[citation!!!]}}

\newcommand{\missref}{\textcolor{red}{[reference!!!]}\ }


%K42
\newcommand{\PC}{$N_{\rm peak}$}
\newcommand{\BIC}{$N_{\rm BI}$}
\newcommand{\PAPR}{$R_{\rm p/>p}$}

\newcommand{\PCR}{$R_{\rm peak}$}


%Pd

\newcommand{\gline}{$\gamma$-line}
\newcommand{\glines}{$\gamma$-lines}


\newcommand{\gray}{$\gamma$-ray}
\newcommand{\grays}{$\gamma$-rays}


\newcommand{\bray}{$\beta$-ray}
\newcommand{\brays}{$\beta$-rays}

\newcommand{\betas}{$\beta$'s}


%general

\newcommand{\tab}{\textcolor{brown}{Tab.~}}
\newcommand{\eq}{\textcolor{brown}{Eq.~}}
\newcommand{\fig}{\textcolor{brown}{Fig.~}}
\renewcommand{\sec}{\textcolor{brown}{Sec.~}}
\newcommand{\chap}{\textcolor{brown}{Chap.~}}


 \newcommand{\fn}{\iffalse \fi} %footnote explaination
 \newcommand{\tx}{\iffalse \fi} %text explaination
 \newcommand{\txe}{\iffalse \fi} %text extended explaination
 \newcommand{\sr}{\iffalse \fi} %section reference explaination
% \renewcommand{\cr}{\iffalse \fi} %citation reference explaination
